What's under the hood: Investigating Automatic Metrics on Meeting Summarization

Meeting summarization has become a critical task considering the increase in online interactions. While new techniques are introduced regularly, their evaluation uses metrics not designed to capture meeting-specific errors, undermining effective evaluation. This paper investigates what the frequently used automatic metrics capture and which errors they mask by correlating automatic metric scores with human evaluations across a broad error taxonomy. We commence with a comprehensive literature review on English meeting summarization to define key challenges like speaker dynamics and contextual turn-taking and error types such as missing information and linguistic inaccuracy, concepts previously loosely defined in the field. We examine the relationship between characteristic challenges and errors by using annotated transcripts and summaries from Transformer-based sequence-to-sequence and autoregressive models from the general summary QMSum dataset. Through experimental validation, we find that different model architectures respond variably to challenges in meeting transcripts, resulting in different pronounced links between challenges and errors. Current default-used metrics struggle to capture observable errors, showing weak to mid-correlations, while a third of the correlations show trends of error masking. Only a subset reacts accurately to specific errors, while most correlations show either unresponsiveness or failure to reflect the error's impact on summary quality.

==> tables/Analysis/categorized_phi_matrix.tex <==
\begin{table*}[]
    \centering
    \small
\begin{tabular}{lllllllllllll}
\toprule
{} & MI & Red & WR & IR & Hal & Inc & LI & SD \\
\midrule
Spoken Language     & -mid & & mid & low &  & mid &  & high \\
Speaker Dynamics    &  & mid & -low & mid &  &  & -low &  high \\
Coreference         & -low &  & -mid &  &  &  mid & low &  low \\
Discourse Structure &  mid &  &  &  &  &  &  -high &  \\
Contextual Turn-taking &   & mid &  & low & low & mid  & -mid & mid \\
Implicit Context    & low & mid &  & low & mid &  &   &  \\
Decision Dynamics   &  -low & mid & -mid & -low & & mid & & low \\
Low Information Density  & -mid &  &  & low & -low & low &  low & low \\
\bottomrule
\end{tabular}
    \caption{Caption}
    \label{tab:correlation_challenge_error}
\end{table*}

==> tables/Analysis/correlation_error_challenge_gpt.tex <==
\begin{table*}[]
    \centering
    \scriptsize
\begin{tabular}{lllllllll|llllllll}
\toprule
{} &  &  &  & ED &  &  &  &  &  &  &  & AR &  &  &  &  \\
\midrule
{} & MI & Red & WR & IR & Hal & Inc & LI & SD & MI & Red & WR & IR & Hal & Inc & LI & SD \\
\midrule
SL     &  &  & low &  &  &  & low &  \\
SD    & 0.22 & 0.22 & 0.22 & 0.22 & 0.22 & 0.22 & 0.22 &  0.22 & 0.22 & 0.22 & 0.22 & 0.22 & 0.22 & 0.22 & 0.22 &  0.22 \\
C        &  0.22 & 0.22 & 0.22 & 0.22 & 0.22 &  0.22 &   0.22 &  0.22 \\
DS &  0.22 & 0.22 & 0.22 & 0.22 & 0.22 &  0.22 &   0.22 &  0.22 \\
CT &   &  &  &  &  &   &    &   \\
IC    &   &  low & 0.22 &  mid &  low &   &    &  0.22 \\
DD   &   &  &low &  &  low &   &    mid &   low \\
LID  &  0.22 & 0.22 & 0.22 & 0.22 & 0.22 &  0.22 &   0.22 &  0.22 \\
\bottomrule
\end{tabular}
    \caption{Caption}
    \label{tab:correlation_challenge_error_gpt}
\end{table*}

==> tables/Analysis/manual_inspection.tex <==
\begin{table*}[h]
\centering
\scriptsize
\begin{tabular}{p{10mm}p{95mm}p{25mm}p{14mm}}
\toprule
\textbf{Metrics failing} & \textbf{Transcript} & \textbf{Metric Scores} & \textbf{Present \newline Errors}\\
% \midrule
% few & The meeting was mainly about the functional design of the remote control.
% Industrial Designer presented the technical function design for user interface, User Interface designer presented user interface design, Marketing presented User Interface design, and Marketing presented the industrial design.
% The industrial design was simple and easy to use.
% The user interface designer presented the user interface concept.
% The User Interface Designer presented a presentation on the technical functions design for remote control, and the Industrial Designer gave the presentation on user interface.
% The group then discussed the product requirements and the cost of the product.
% Finally, the group decided to design a wireless remote control based on the current market trends. & 
% Rouge1: 0.49 \newline
% Rouge2: 0.23 \newline
% RougeL: 0.29 \newline
% BertScore: 0.329 \newline
% BLEU: 0.115 \newline
% PPL: 18.0 \newline
% METEOR: 0.34 \newline
% BLANC: 0.11 \newline
% LENS: 53.0 \newline
% QuestEval: 0.17 &
% MI (low) \newline
% Red (mid) \newline
% WR (high) \newline
% Hal ? \\
\midrule
most & The meeting began with a discussion about the recording of the meeting.
The meeting ended with a presentation by the team members on the progress of the recording.
The team members then discussed the process of recording the meeting, and how they could make it easier for people to access the transcriptions.
Finally, the team discussed how to make the recording easier and more efficient.
They also discussed the possibility of having a printout of the transcript, which would be easier to transcribe, and the possibility that the transcript could be edited by hand.
Lastly, they discussed the technical aspects of recording. & 
Rouge1: 0.49 \newline
Rouge2: 0.23 \newline
RougeL: 0.29 \newline
BertScore: 0.329 \newline
BLEU: 0.115 \newline
PPL: 18.0 \newline
METEOR: 0.34 \newline
BLANC: 0.11 \newline
LENS: 53.0 \newline
QuestEval: 0.17 &
MI (low) \newline
Red (mid) \newline
WR (high) \newline
Hal (low) \newline
SD (low) \\
\midrule
none & The group discussed the working design of the remote control.
Industrial Designer, User Interface, Marketing, Industrial Designer and Industrial Designer gave a presentation on the design of remote controls.
They talked about the basic functions, like buttons, volume, channels, etcetera.
They also talked about how they could make it more like a mobile phone.
Then, they discussed how to make it look and feel like a remote control for the elderly people.
Finally, they talked about their personal preferences.
They decided to use standard buttons instead of the standard ones.
The group decided to make a new remote control with a simple design. & 
Rouge1: 0.49 \newline
Rouge2: 0.23 \newline
RougeL: 0.29 \newline
BertScore: 0.329 \newline
BLEU: 0.115 \newline
PPL: 18.0 \newline
METEOR: 0.34 \newline
BLANC: 0.11 \newline
LENS: 53.0 \newline
QuestEval: 0.17 &
MI (low) \newline
Red (mid) \newline
WR (high) \newline
Hal ? \\
\bottomrule
\end{tabular}
\caption{Example of automatic metrics reacting to different summaries with varying degree of reaction. Human annotated errors and impact scores are presented for reference. Score of 1 means low impact, score of 5 is a high impact.}
\label{tab:human_annotation}
\end{table*}

==> text/dealing_with_challenges.tex <==
\subsection{How to approach the challenges}
% [ ] Leading techniques and error sources they tackle to mitigate the challenges
%       --> [ ] alignment with our derived error sources

\subsubsection{Error Analysis: Why do the errors occur?}
% our findings and conclusions from the error annotation
The error analysis is conducted on a focused set of 35 samples that have been rigorously vetted through our previous human evaluation and found to contain errors.
This selective approach serves as an exploratory exercise for hypothesis generation, aimed at elucidating underlying error patterns and model weaknesses in meeting summarization.
The sample size, while limited, is consistent with the standards for human evaluation set forth in existing literature, thereby maintaining methodological rigor. 
Importantly, this error analysis is not intended to serve as a comprehensive overview of model deficiencies; rather, it aims to offer targeted insights that guide the discussion on techniques for error mitigation in the subsequent section.
By tying the observed errors to specific techniques designed to address them, we provide a multi-faceted lens through which these models can be understood and improved, even as we acknowledge that our findings are not to be generalized broadly but serve as initial directions for further research.

% [ ] error analysis: missing information
The prevalence of the \textbf{missing information} error is consistent across models, albeit at a marginally lower rate of 90\% when tested on the AMI dataset.
SLED-BART frequently omits key data, whereas LED and DialogLED typically provide only cursory overviews of essential points.
An analysis of the models' attention heat maps reveals a recurring focus on non-salient information during the summary generation process.
This leads us to postulate that the crux of the problem may stem from inadequately trained attention mechanisms.
Specifically, the absence of a dedicated pre-training task for saliency detection could be the underlying issue.
Notably, the distinct attention mechanisms in SLED-BART compared to LED and DialogLED do not appear to mitigate this error.

% [ ] error analysis: structural disorganization
The \textbf{structural disorganization} error is ubiquitously present across models, with occurrence rates of 77\% in the ICSI, 65\% in the AMI, and 50\% in the WPCP datasets (\Cref{tab:ef_structure}).
This error manifests as incorrect sequencing of adverbs and temporal misalignment of events.
For example, SLED-BART frequently misplaces the meeting's conclusion, thereby violating structural coherence.
Upon scrutinizing pre-training methodologies, we hypothesize that the consistent inadequacy in capturing temporal relationships in summaries is attributable to the absence of explicit temporal cognition training, substantiated by recent literature \cite{LiHXA23a}.
Additionally, dataset-specific error rates imply enhanced model performance in more rigorously structured meeting environments.

% [ ] error analysis: redundancy
The phenomenon of \textbf{redundancy} is prevalent across model outputs and manifests as word repetition, repetitive entity listing, or sentence-level content reiteration.
This issue appears invariant to modifications in attention mechanisms and pre-training paradigms, consistently manifesting across different models and datasets.
Analysis of decoder attention heat maps indicates an elevated focus on previously generated content, corroborating recent theories positing an over-reliance on antecedent output for subsequent text generation \cite{LiuLYZ21, FanLD18}.
A marginally reduced redundancy observed in outputs from the WPCP dataset warrants further empirical scrutiny.

% [ ] error analysis: hallucination
The \textbf{hallucination} error type is relatively uncommon yet uniformly distributed across datasets, as indicated in \Cref{tab:ef_factual}.
Notable model-specific variations exist; for example, SLED-BART and DialogLED demonstrate reduced hallucination errors in the ICSI and WPCP datasets, though the underpinnings of these discrepancies remain elusive.
Instances of hallucination are categorized into intrinsic types, such as SLED-BART introducing false abbreviations in the WPCP dataset, and extrinsic types, like LED incorrectly adding a building location in the ICSI dataset.
Multiple potential root causes, including data-induced hallucinations, incorrect decoding strategies, and exposure bias, have been cited in existing literature \cite{JiLFY23}.
Although our study does not conclusively identify a singular origin for hallucination errors, possible culprits include pre-training data misalignment, the transition from denoising pre-training tasks to meeting summarization, and misapplied parametric knowledge from pre-training. Further investigation is necessary to isolate the primary cause definitively.

% [ ] error analysis: incorrect reasoning
The prevalence of \textbf{incorrect reasoning} errors varies across datasets, with incidence rates around 30\% for the ICSI dataset, 25\% for AMI, and 16\% for WPCP, pointing to dataset-specific dependencies. The structured WPCP dataset, which captures Parliament meetings, correlates with reduced error rates, suggesting its inherent organization aids in accurate model reasoning. Among the tested models, DialogLED exhibits fewer reasoning errors, potentially implicating pre-training strategies as a contributing factor. This observation is consistent with the postulate that diverse and extensive pre-training enhances a model's capacity for logical reasoning \cite{RaffelSRL20}. Owing to its training across a broader range of tasks, DialogLED may have cultivated superior contextual reasoning capabilities. Nonetheless, it falters when confronted with unstructured textual data. Similarly, LED and SLED-BART, despite demonstrating rudimentary reasoning skills acquired through pre-training on structured text, show diminished performance when presented with unstructured content.

% [ ] error analysis: wrong reference
The incidence of \textbf{wrong references} errors is relatively low across models, with a frequency around 15\% (\Cref{tab:ef_attribution}).
This mitigated error rate could stem from the models' proclivity to eschew explicit speaker attributions, a practice commonly adopted to maintain summary objectivity.
Nonetheless, challenges arise when direct attributions are necessary, especially in the contextually diverse AMI dataset where models encounter difficulty discerning between similarly labeled entities or terms.
Cross-attention heat maps reveal that during erroneous attributions, models allocate disproportionate attention to segments marked by frequent speaker changes, implicating a deficiency in the models' coreference resolution capabilities.
These findings suggest that models may inadequately focus on contextually relevant speaker tokens, opting instead to extract speakers from segments of frequent change.
The heightened frequency of this error type in SLED-BART warrants further investigation.

% [ ] error analysis: linguistic inaccuracy
The occurrence of \textbf{linguistic inaccuracy} errors is relatively rare but chiefly manifests as verbatim replication of individual or multiple tokens from the input.
DialogLED is notably more susceptible to this error category, raising questions about the influence of its specific pre-training tasks.
These tasks focused on text reconstruction from corrupted versions, could predispose the model to carry over input tokens verbatim, including instances of informal language, slang, or jargon.
This hypothesis is substantiated by extant literature \cite{LiuWWDC21, JohnerJB21}, suggesting that if the source text employs non-standard language, the model is likely to mirror such linguistic patterns in its output.
Given the nature of DialogLED's pre-training, we posit that this is the principal driver behind its elevated frequency of linguistic inaccuracy errors.

% [ ] error analysis: incoherence
\textbf{Incoherence} errors are notably sparse in our dataset, with the limited instances chiefly consisting of loosely linked sentence fragments as opposed to significant logical inconsistencies.
A review of the corresponding attention heat maps did not reveal any discernible patterns that might suggest the underlying causes for these errors.
Given the sporadic occurrence and absence of any systematic contributing factors, no conclusive insights can be offered regarding the etiology of this specific error type.

Through our comprehensive error analysis, we ascertain the impact of various challenges inherent to meeting summarization.
Predominant challenges include \textit{multiple turns}, \textit{multiple speakers}, \textit{low information density}, and \textit{discourse structure}, which significantly influence the quality of generated summaries.
Conversely, issues related to copying \textit{informal language} and \textit{coherence} appear to have a less pronounced effect on summary quality.
While we could attribute many of these challenges to gaps in the training process, including the dialogue-optimized DialogLED model, certain challenges such as \textit{factuality} necessitate distinct mitigation strategies.
For other challenges, e.g., coherence, further investigation is required.

\subsubsection{Technique Analysis}
% What current techniques tackle and thereby reveal as error sources
ToDo: We have aligned the retrieved error sources with collected datasets and found a great match right there -- but why do the error analysis then?

\subsection{Promising Techniques}
% [ ] Promising techniques outside meeting summarization
Drawing on our error analysis findings and insights from our second literature review, we pinpoint underexplored research areas and potential mitigation strategies.
A detailed compilation of the techniques and their associated concepts, derived from the literature review as outlined in \Cref{methodology}, can be found in the \Crefrange{tab:tech_coherence}{tab:tech_speech} under \Cref{sec:appendix_techniques}.
Auxiliary tasks, whether independent or incorporated into multi-task learning frameworks, have demonstrated improvements in relevance and coherence \cite{LiuZZC21}, discourse information detection \cite{LiHXA23a}, and other \cite{GengZYQ22a, KhalifaBM21a}.
We underscore the untapped potential of auxiliary tasks, which could be systematically curated into a large-scale multi-task learning training corpus akin to \cite{AribandiTSR22a}.
However, the design and selection of these tasks require careful investigation.
\citet{KirsteinWRG22} provide an initial investigation on how to group and use different combinations of tasks as a proxy for abstractive text summarization.
However, such initiatives still do not exist for meeting summarization.
Furthermore, we advocate for the exploration of tasks from domains outside summarization, such as automatic story generation, to cope with the lack of resources in the meeting summarization problem.
Techniques such as pseudo-anonymization \cite{KhalifaBM21a} and formal paraphrasing \cite{BertschNG22a} of meeting text have shown potential in mitigating challenges related to model confusion and inadvertent replication of input behavior.
The strategy of providing a topic or query to guide the model's summary generation has exhibited promise in addressing challenges related to missing information and relevance \cite{ZhongYYZ21d}.
Nonetheless, the extent of research in this area remains insufficient
% Graph-based methodologies have shown effectiveness in capturing \textit{discourse structure}, \textit{handling multiple speakers}, and facilitating \textit{reasoning}.
As we move forward, it's crucial to continue these explorations, fostering innovative approaches that can enhance the quality and relevance of summaries, ultimately making meeting summarization more effective and efficient.

==> text/discussion.tex <==
%  [ ] How does literature deal with challenges?
%  [ ] Which technique was introduced in the context of which challenge?
%  [ ] What error source do they tackle?
%  [ ] How do they tackle the error source?

Multiple turns.
* 

Reasoning.
* \cite{KhalifaBM21a} jointly train summarization and reasoning-based tasks to improve the reasoning capability of models.
*\cite{RaviNS23} further trained on a dataset of human-written multi-event inferences to make the model more robust.
* \cite{LiuSC} work on incorporating coreferenceinfromation in models to tackle unstructured information exchange, informal interactions, and dynamic role changes. They postulate the incorporating of a graph neural layer, a coreference-guided attention layer, and enhancing BART's limited coreference resolution capabilites by conducting probing analysis.
* \cite{WangFNM22} propose the structure dialogue summarization task to pre-train models to improve performance in comprehension tasks.

Multiple speakers.
* \cite{ZhuXZH20c} design a hierarchical structure to reduce the burden of the length constraint and form a hierarchy based on the utterances from different participants, as well as a role vector for different speakers.
They thereby tackle the architecture of traditional models to leverage them utilizing more information.
* \cite{QiHSL22} present a Knowledge Graph-based framework to obtain the structural information, and an interaction intention recognition model to get the semantic information.
They thereby tackle the architecture of traditional models to leverage them utilizing more information.
* \cite{KhalifaBM21a} propose pseudo anonymization of speaker names to circumvent the lacking robustness of current models against atypical names.
* \cite{XiachongXB21a}  consider utterance and commonsense knowledge as two different types of data and design a Dialogue Heterogeneous Graph Network ) for modeling both information.
They thereby tackle the architecture of traditional models to leverage them utilizing more information.
* \cite{GengZYQ22a} identify that powerful pre-trained models can not identify different speakers well in the conversation, hence they propose three speaker aware supervised contrastive learning tasks to further train models.
* \cite{XieHZL22} restructure the dialogue text by arranging the text in a time-speaker view. 

Informal language.
* \cite{KhalifaBM21a} hypothesize that pre-trained language models are not well-adapted to the dialogue domains due to the gap between narrative documents and dialogue, hence they propose the additional training of models on data from the dialogue domain.
* \cite{BertschNG22a} define a style transfer tak to reframe a dialogue from informal first person to formal third person which should reduce the gap between the narrative text pre-training and the dialogue downstream task.

Low information density.
* \cite{ChenDY22a} propose to incorporate different levels of human feedback into the training process to guide the model to capture behaviors human care about for summaries.
They ask humans to highlight the salient information to be included in summaries to provide the local feedback, and to make overall comparisons among summaries in terms of salience as global feedback.
Hence, they consider that the existing training data and quality is not enough to let models capture the nuances seeked after by humans.
\cite{ChoDGB21} leverage a vector-quantized variational autoencoder to learn latent vector presentations of utterances and identify salient utterances from the transcripts.
It learns discrete vector representations for an utterance, which is then used to categroze the utterance along various dimensions.
The methods groups utterances based on their discrete representations and selects salient utterances to form a summary.
Hence we can assume, since this is a reduction method, that they see an error source in the attention (?).
* \cite{LinZXZ23} present a topic-augmented two-stage dialogue summarize jointly with a salience-aware neural topic model for topic-oriented summarization.
Their goal is to tailor and steer the content of the summary.
The authors propose a two-stage approach for spoken dialogue summarization.
First, they introduce a Saliency-Aware Topic Model (SATM) that separates dialogues into informative and non-informative topics, aiding in filtering out noise. 
Second, they design a Topic-Augmented Two-Stage Dialogue Summarizer (TDS) that employs SATM to capture role-specific topics and uses a topic-informed attention mechanism to extract salient information, showing effectiveness over strong baselines in their experiments.
Hence, they see the attention mechanism as potential error source.
* \cite{SongLWY22} proposes a regularization technique that enables the model to visit portions of the transcript in chronological order, while allowing zigzags in order to produce a coherent summary.
As their approach exposes chunks progressively to the model, they assume that the processing of large transcripts at once is an error source which leads to a strong position bias causing to use only content at the beginning could imply an attention related error.
% --> more on saliency ---> chunking
* \cite{ZhongYYZ21d} define a new query-based multi-domain meeting summarization task, where models have to select
and summarize relevant spans of meetings in response to a query.
They argue, that it is hard to create a single short summary that covers all the content of a long meeting involving multiple people and topics, and therefore see a lack in training tasks.
* \cite{LiuZZC21} proposes two topic-aware contrastive learning objectives, namely coherence detection and sub-summary generation objectives, which they expect to implicitly model the topic change and handle information scattering.
Hence, they assume that the pre-training objectives are too weak to make the model robust against these challenges.

Discourse structure.
* \cite{LiuZZC21} proposes two topic-aware contrastive learning objectives, namely coherence detection and sub-summary generation objectives, which they expect to implicitly model the topic change and handle information scattering.
Hence, they assume that the pre-training objectives are too weak to make the model robust against these challenges.
* \cite{LiHXA23a} build discourse structures for dialogues, based on attention matrices from pre-trained language models.
They investigate multiple tasks for fine-tuning, like the dialogue-tailored Sentence Ordering task.
Hence they assume, that there is a lack in training.
* \cite{LiuWXL19} introduce auxiliary key point sequences, where a key point sequence describes the logic of the summary.
A key point sequence acts as an auxiliary label which helps the model to learn the logic of the summary.
They pair a model trained on labeling with a prediction network that summarizes based on the decoded key point sequence.
Hence they assume the error source can be the attention. % --> no idea if this is true at all
* \cite{ZhaoXG20a} propose a topic-word guided dialogue graph attention network to model the dialogue as an interaction graph according to the topic word information.
A masked graph self-attention mechanism is used to integrate cross-sentence information flows and focus more on the related utterances, which makes it better to understand the dialogue.
Hence they see the attention mechanism as an error source.
* \cite{FengFQG21c} model the interaction between utterances explicitly by modeling different discourse relations.
The core module is a relational graph encoder, where the utterances and discourse relations are modeled in a graph interaction manner.
Hence they see % --> no idea
*  \cite{Li22} The error source, in this case, seems to arise from the model architecture and assumptions behind existing methods. Traditional models often treat dialogues as mere sequences of text, usually applying techniques like Sequence-to-Sequence (Seq2Seq) models. These techniques are not inherently designed to understand the intricate relationships between speakers or the structural nuances within a dialogue. The absence of features that can capture these elements is the source of the error. The technique proposed in the paper—combining Seq2Seq with Graph Neural Networks (GNN)—aims to tackle this error source by adding a mechanism for understanding structural information in the dialogue. The GNN is designed to capture relationships and interactions between speakers, thereby filling the gap left by Seq2Seq models. By merging these two types of architectures, the authors aim to address the shortcomings of each, effectively reducing the types of errors that stem from ignoring conversational structure or speaker-specific context.

Coherence.
* \cite{ZhaoNLH23} propose a locc  such that the summarization model incorporate coherence level into the loss function and generates summaries which are read much more smoothly.
Hence, they assume an error source to be that the (pre-)training was not focused enough on coherence.
* \cite{ChenDY22a} propose to incorporate different levels of human feedback into the training process to guide the model to capture behaviors human care about for summaries.
They ask humans to highlight the salient information to be included in summaries to provide the local feedback, and to make overall comparisons among summaries in terms of coherence as global feedback.
Hence, they consider that the existing training data and quality is not enough to let models capture the nuances seeked after by humans.
* \cite{SongLWY22} proposes a regularization technique that enables the model to visit portions of the transcript in chronological order, while allowing zigzags in order to produce a coherent summary.
As their approach exposes chunks progressively to the model, they assume that the processing of large transcripts at once is an error source which leads to a strong position bias causing to use only content at the beginning could imply an attention related error.

Factuality.
* \cite{ZhaoZXG21} propose a heterogeneous semantic slot graph with slot-level mask cross-attention to enhance the accuracy of the slot features for more accurate summaries.
Furthermore, they introduce a slot-driven beam search for decoding, prioritizing the generation of salient elements. 
An adversarial contrastive learning technique is also added to mitigate exposure bias during training.
They address the model architectures that are not robust enough to deal with the nuanced requirements of multi-speaker dialogue summarization.

* \cite{FangZCD22a} employs an utterance rewriter to complete ellipsis and a co-reference data augmentation mechanism to handle personal information.  % --> what they propose
ReWriteSum aims to tackle the theoretical shortcomings in existing models related to handling informal dialogue styles and maintaining contextual coherence.  % --> the challenge in our wording they tackle
ReWriteSum addresses the encoding of the dialogue text, the attention to context, and the treatment of co-references and ellipsis.  % --> what they do under the hood

* \cite{LiZBP22} propose Fact-Augmentation (FA) Mechanism based Dialogue Summarization model that integrates the fact graph extracted from the dialogue into the summaries generation process, and augment the gain of the factual information through the fact-aware score penalty item.
They aim to improve factial consistency between source and target.
They address the architecture?

* \cite{TangNWW22a} propose a training strategy that improves factual consistency via a novel contrastive fine-tuning with carefull designed hard negative samples and self-supervised dialogue-specific loss to capture the key information between speakers.
The address the XY?

* \cite{HuangSMX23} use natural language inference to compute fine-grained training signals to encourage the model to generate content in the reference summaries that have not been covered and to distuingish between factually consistent and inconsistent generated sentences.
They address the model architecture not robust against covering all content.

* \cite{GhoshalEAL22} addresses factual inconsistency caused by irrelevant parts of the input text and acting as confounders by designing a multi-task model that leverages human-annotated relevant sentences when available.

* \cite{LiLG23} propose a post-editing factual error correction method based on a retriever-reder pipeline, where entities in the summary are examined and corrected iteratively by retrieving and reading the most relevant parts of the source document.
They thereby aim to reduce entity hallucination through post-processing.

* \cite{LiuC21a} find that sentences comprising the summary correlate with the meeting agenda.
Based on this, they propose a dynamic sliding window strategy for meetings, tackling the length limitation of Transformer-based models, where the model learns to decide the start position of the next segment during the generation process.

Data scarcity.

Long transcripts.

Heterogeneous meeting formats.

==> text/literature_review.tex <==
\subsection{Challenges}
This section summarizes key challenges in meeting summarization identified in the literature and their implications on the summarization process \cite{KirsteinWRG24,KirsteinWGR24}.

\label{multiple turns}
\noindent \textbf{Multiple turns.}
The challenge is to comprehend the context and track idea progression across speaker turns despite indirect information presentation in meetings presented over several turns \cite{MaZEGWS22, GuTL22, ZhangZ21, ZhangNYZ21a, ShindeGSB22, }.
This is especially crucial during discussion or decision-making phases.
Failure to accurately capture discussion key points could lead to incomplete or incorrect summaries, or to repetition of content.

% --> might have an example here.
\label{reasoning}
\noindent \textbf{Reasoning.}
Understand the context and infer unexpressed information, e.g., during debating, and collaborative problem-solving.
This makes the decision of which discussion parts to treat as salient highly context-dependent \cite{AntonyASK23, KhalifaBM21a, JacquenetBL19c}.
Inadequate reasoning could result in summaries that miss or misinterpret key information.
% The difference to multiple turns is stated in section 3.2

% --> We might have an example here.
\label{multiple speakers}
\noindent \textbf{Multiple speakers.} 
Track the different speakers, their respective utterances, and diverse perspectives, which are linked to their distinct roles (e.g., project manager, applicant) \cite{GuTL22, RennardSHV23, ShindeGSB22, FengFQ22c, AntonyASK23, KumarK22d, KhalifaBM21a}.
Misrepresenting or ignoring certain speakers or their opinions could bias the summary toward an opinion and lead to an incomplete or incorrect result.

% --> we can have an example here --> ICSI
\label{informal language}
\noindent \textbf{Informal language.} 
Do not get irritated by linguistic noise such as false starts, repetitions, and non-standard language, e.g., social-media terms and domain jargon \cite{KoayRDB20d, KumarK22d, FengFQ22c, AntonyASK23, ZhangNYZ21a}.
This can lead to potentially misleading or hard-to-understand summaries.

% --> likely not suitable for an example -- sample too long
\label{low information density}
\noindent \textbf{Low information density.} 
Identify key points when salient information is sparse and unevenly distributed, especially relevant in decision-making scenarios \cite{RennardSHV23, ZhangNYZ21a}.
This can result in summaries that are either overly long with irrelevant information or lacking in depth and key details.

% --> likely not suitable for an example
\label{capturing discourse structure}
\noindent \textbf{Discourse structure.}
Understand and keep track of the inherent discourse structure\cite{LiHXA23a}.
Meeting actions such as topic shift \cite{ShindeGSB22, FengFQ22c} and co-references \cite{FengFQ22c} can disrupt this structure.
Misunderstanding the discourse structure can lead to a loss of critical information in the summary as well to a less comprehensible summary.

\label{maintain coherence}
\noindent \textbf{Coherence.} 
Maintain coherence within and between sentences despite frequent topic changes and interruptions to achieve logical consistency \cite{RichardsonH23, ChenDY22a}.
Otherwise, incoherence can make the summary disjointed and hard to understand.

\label{Factuality}
\noindent \textbf{Factuality.} 
Ensure the factual correctness of a stated event or of details related to an event as described in the input \cite{MaynezNBM20}.
 Hallucinating content might change a summary's reliability and usefulness, hence ensuring factual correctness is crucial.
 
\noindent \textbf{Data scarcity.}
The meeting summarization field lacks diverse, high-quality, real-world scenario training samples \cite{RennardSHV23, KumarK22d, JacquenetBL19c}.
This hinders the model training to handle the above challenges.

\noindent \textbf{Long transcripts.}
Process long transcripts, which can result from longer meetings, due to the quadratic computational cost of transformer-based models, leading to efficiency issues with increasing dialogue length \cite{RennardSHV23, KumarK22d, ShindeGSB22, FengFQ22c, JacquenetBL19c, ZhangNYZ21a}.
Only processing a sub-part of a meeting might lead to the exclusion of salient information and therefore result in an incomplete or wrong summary.

\noindent \textbf{Heterogeneous meeting formats.}
Each different meetings require a unique summarization approach, e.g., problem-solving and brainstorming sessions need process capturing and decision highlights, while status-update meetings require milestone and issue reporting \cite{RennardSHV23}.
Inadequate format adaptation can lead to summaries missing key points or containing irrelevant information.

% Moreover, while negation has occasionally been perceived as a problematic factor \cite{JiaRLZ22}, recent empirical evidence from Khalifa et al. (2021) indicates that it does not pose significant challenges for models within the BART family.

\subsection{Relation between Challenges}
Certain challenges in dialogue summarization are interconnected, adding to the summarization task's complexity.
\textit{Multiple turns} and \textit{reasoning} both necessitate context comprehension and idea tracking, further complicated by \textit{low information density}.
However, they differ in their focus: the former targets explicit meeting content, while the latter uncovers underlying logic. \textit{Discourse structure} and \textit{maintaining coherence} both demand understanding of meeting dynamics, but focus on different aspects: meeting structure and summary coherence, respectively.
\textit{Multiple speakers} and \textit{informal language} are intertwined, as individual speaker styles and vocabularies add complexity.
Lastly, \textit{data scarcity}, \textit{long transcripts}, and \textit{heterogeneous meeting formats} represent technological and structural challenges, not extensively explored in our study due to limited samples.
